Simultaneous Finite Automata: An Efficient Data-Parallel Model for Regular Expression Matching

Automata play important roles in wide area of computing and the growth of multicores calls for their efficient parallel implementation. Though it is known in theory that we can perform the computation of a finite automaton in parallel by simulating transitions, its implementation has a large overhead due to the simulation. In this paper we propose a new automaton called simultaneous finite automaton (SFA) for efficient parallel computation of an automaton. The key idea is to extend an automaton so that it involves the simulation of transitions. Since an SFA itself has a good property of parallelism, we can develop easily a parallel implementation without overheads. We have implemented a regular expression matcher based on SFA, and it has achieved over 10-times speedups on an environment with dual hexa-core CPUs in a typical case.

==> img/par_dfa_org.tex <==
\begin{algorithmic}
\REQUIRE DFA ${\cal D} = (Q_d, \Sigma, \delta_d, \{q_0\}, F_d)$, number of threads $p$ , word $w = \sigma_1\sigma_2\cdots\sigma_n$\\
$w = \sigma_{11}\cdots\sigma_{1m_1}\sigma_{21}\cdots\sigma_{2m_2}\cdots\sigma_{p1}\cdots\sigma_{pm_p}$
for simplicity, $p$ is factor of $n$ and power of two
\ENSURE $q_{final}$ is destination $q_0 \xrightarrow[{\cal D}]{w} q_{final}$
\FORALL{$i = 1 \to p$ {\bf parallel}}
\FORALL{$q \in Q_d$}
\STATE $T_i[q] = q$
\ENDFOR
\STATE $base \leftarrow n/p * (i - 1)$
\FORALL{$j = 1 \to n/p$}
\FORALL{$q \in Q_d$}
\STATE $T_i[q] \leftarrow \delta(T_i[q], \sigma_{base+j})$
\ENDFOR
\ENDFOR
\ENDFOR
\STATE
\STATE $reduction \leftarrow 1$
\WHILE{$reduction \neq p$}
\STATE $reduction \leftarrow reduction * 2$
\FORALL{$r = reduction, reduction*2, \cdots \to p$ {\bf parallel}}
\FORALL{$q \in Q_d$}
\STATE $T_r[q] \leftarrow T_r[T_{r-reduction/2}[q]]$
\ENDFOR
\ENDFOR
\ENDWHILE
\STATE
\STATE $q_{final} \leftarrow T_r[q_0]$
\end{algorithmic}

